Lexical Co-occurrence, Statistical Significance, and Word Association

Lexical co-occurrence is an important cue for detecting word associations. We present a theoretical framework for discovering statistically significant lexical co-occurrences from a given corpus. In contrast with the prevalent practice of giving weightage to unigram frequencies, we focus only on the documents containing both the terms (of a candidate bigram). We detect biases in span distributions of associated words, while being agnostic to variations in global unigram frequencies. Our framework has the fidelity to distinguish different classes of lexical co-occurrences, based on strengths of the document and corpuslevel cues of co-occurrence in the data. We perform extensive experiments on benchmark data sets to study the performance of various co-occurrence measures that are currently known in literature. We find that a relatively obscure measure called Ochiai, and a newly introduced measure CSA capture the notion of lexical co-occurrence best, followed next by LLR, Dice, and TTest, while another popular measure, PMI, suprisingly, performs poorly in the context of lexical co-occurrence.

==> discussion.tex <==
\section{Discussion}

Threshold span needs discussion. Essentially we say that, it is reasonable to believe that all
occurrences with span less than the threshold value can plausibly be motivated, while all
occurrences with span greater than the threshold span are probably arbitrary. This notion applies to
all co-occurrence based measures, not just the CSR



==> figures.tex <==

\begin{figure}
  \begin{center}
    \begin{tabular}{cc}
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{simExpiryTimeDeltaS}} &
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{simExpiryTimeEffectW}} \\
    \end{tabular}
    \caption{Effect of span threshold on correlation of significance ratio (CSR) with human judgement}
    \label{expiryTimeDeltaFigs}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
     \addtolength{\tabcolsep}{-9pt}
    \begin{tabular}{ccc}
	\resizebox{60mm}{!}{\includegraphics[angle=-90]{simScatterPlot}} &
	\resizebox{60mm}{!}{\includegraphics[angle=-90]{simScatterPlot1}} &
      	\resizebox{60mm}{!}{\includegraphics[angle=-90]{simScatterPlot2}} \\	
    \end{tabular}
    \caption{Variation in correlation of various co-occurrence measures with human judgement}
    \label{expiryTimeFigs}
  \end{center}
\end{figure}


%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/esslli/esslliExpiryTimeEffectS}
%  \caption{esslliExpiryTimeEffectS.png}
%\end{figure}
%
%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/esslli/esslliExpiryTimeEffectW}
%  \caption{esslliExpiryTimeEffectW.png}
%\end{figure}
%
%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/rel/relExpiryTimeEffectS}
%  \caption{relExpiryTimeEffectS}
%\end{figure}
%
%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/rel/relExpiryTimeEffectW}
%  \caption{relExpiryTimeEffectW}
%\end{figure}
\begin{comment}
\begin{figure}
  \begin{center}
    \begin{tabular}{cc}
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{simExpiryTimeDeltaW}} &
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{simExpiryTimeDeltaS}} \\
    \end{tabular}
    \caption{Effect of expiry time on correlation of Significance Ratio with Human Judgement}
    \label{expiryTimeDeltaFigs}
  \end{center}
\end{figure}


\begin{figure}
  \begin{center}
    \begin{tabular}{cc}
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{simExpiryTimeEffectW}} &
      	\resizebox{80mm}{!}{\includegraphics[angle=-90]{simExpiryTimeEffectS}} \\
    \end{tabular}
    \caption{Effect of expiry time on correlation of different measures with Human Judgement}
    \label{expiryTimeFigs}
  \end{center}
\end{figure}

\end{comment}


==> tables.tex <==
\begin{table}
\small \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | c c c c |}
\hline
Measure	&	Similarity	&	Relatedness	&	WordSim353	&	ESSLLI	\\ 
\hline
CSR & 0.66 & 0.62 & 0.60 & 0.44 \\
PMI & 0.74 & 0.69 & 0.70 & 0.34 \\
LLR & 0.57 & 0.55 & 0.51 & 0.38 \\
Dice & 0.67 & 0.59 & 0.60 & 0.37 \\
Ochiai & 0.69 & 0.64 & 0.63 & 0.46 \\
Jaccard & 0.67 & 0.59 & 0.60 & 0.37 \\
TTest & 0.50 & 0.49 & 0.44 & 0.34 \\
ChiSquare & 0.69 & 0.64 & 0.63 & 0.46 \\
SCI & 0.44 & 0.38 & 0.37 & 0.46 \\
CWCD & 0.64 & 0.53 & 0.56 & 0.36 \\
MCD & 0.69 & 0.57 & 0.62 & 0.37 \\
\hline
\end{tabular}
\caption{ \small Best correlation for each measure}
\label{BestPerformanceTable}
\end{table}


\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (2s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (10w)\end{sideways} & \begin{sideways}Ochiai (1s)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (5w)\end{sideways} & \begin{sideways}CWCD (10w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways} \\
\hline
CSR (2s) & 1.00 & 0.72 & 0.90 & 0.91 & 0.93 & 0.86 & 0.77 & 0.70 & 0.85 \\
PMI (15w) & 0.72 & 1.00 & 0.62 & 0.71 & 0.73 & 0.50 & 0.48 & 0.85 & 0.78 \\
LLR (5w) & 0.90 & 0.62 & 1.00 & 0.95 & 0.94 & 0.98 & 0.85 & 0.66 & 0.74 \\
Dice (10w) & 0.91 & 0.71 & 0.95 & 1.00 & 0.97 & 0.91 & 0.80 & 0.76 & 0.79 \\
Ochiai (1s) & 0.93 & 0.73 & 0.94 & 0.97 & 1.00 & 0.91 & 0.80 & 0.72 & 0.84 \\
TTest (5w) & 0.86 & 0.50 & 0.98 & 0.91 & 0.91 & 1.00 & 0.85 & 0.57 & 0.66 \\
SCI (5w) & 0.77 & 0.48 & 0.85 & 0.80 & 0.80 & 0.85 & 1.00 & 0.73 & 0.58 \\
CWCD (10w) & 0.70 & 0.85 & 0.66 & 0.76 & 0.72 & 0.57 & 0.73 & 1.00 & 0.68 \\
MCD (doclen) & 0.85 & 0.78 & 0.74 & 0.79 & 0.84 & 0.66 & 0.58 & 0.68 & 1.00 \\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for Similarity Dataset}
\label{SimCorrlMatrix}
\end{table}


\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (5s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (15w)\end{sideways} & \begin{sideways}Ochiai (20w)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (5w)\end{sideways} & \begin{sideways}CWCD (5w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways}
 \\
\hline
CSR (5s) & 1.00 & 0.63 & 0.88 & 0.85 & 0.93 & 0.86 & 0.71 & 0.55 & 0.86\\
PMI (15w) & 0.63 & 1.00 & 0.58 & 0.65 & 0.70 & 0.46 & 0.38 & 0.76 & 0.68\\
LLR (5w) & 0.88 & 0.58 & 1.00 & 0.92 & 0.95 & 0.99 & 0.78 & 0.62 & 0.78\\
Dice (15w) & 0.85 & 0.65 & 0.92 & 1.00 & 0.96 & 0.90 & 0.72 & 0.67 & 0.77\\
Ochiai (20w) & 0.93 & 0.70 & 0.95 & 0.96 & 1.00 & 0.92 & 0.74 & 0.65 & 0.85\\
TTest (5w) & 0.86 & 0.46 & 0.99 & 0.90 & 0.92 & 1.00 & 0.79 & 0.54 & 0.73\\
SCI (5w) & 0.71 & 0.38 & 0.78 & 0.72 & 0.74 & 0.79 & 1.00 & 0.71 & 0.6\\
CWCD (5w) & 0.55 & 0.76 & 0.62 & 0.67 & 0.65 & 0.54 & 0.71 & 1.00 & 0.58\\
MCD (doclen) & 0.86 & 0.68 & 0.78 & 0.77 & 0.85 & 0.73 & 0.60 & 0.58 & 1.00\\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for Relatedness Dataset}
\label{RelCorrlMatrix}
\end{table}

\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{| l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (5s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (15w)\end{sideways} & \begin{sideways}Ochiai (20w)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (5w)\end{sideways} & \begin{sideways}CWCD (10w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways} \\
\hline
CSR (5s) & 1.00 & 0.62 & 0.88 & 0.85 & 0.92 & 0.85 & 0.71 & 0.55 & 0.83  \\
PMI (15w) & 0.62 & 1.00 & 0.54 & 0.64 & 0.70 & 0.41 & 0.37 & 0.80 & 0.76  \\
LLR (5w) & 0.88 & 0.54 & 1.00 & 0.92 & 0.94 & 0.98 & 0.79 & 0.55 & 0.74  \\
Dice (15w) & 0.85 & 0.64 & 0.92 & 1.00 & 0.96 & 0.89 & 0.73 & 0.67 & 0.77  \\
Ochiai (20w) & 0.92 & 0.70 & 0.94 & 0.96 & 1.00 & 0.90 & 0.75 & 0.65 & 0.84  \\
TTest (5w) & 0.85 & 0.41 & 0.98 & 0.89 & 0.90 & 1.00 & 0.80 & 0.46 & 0.67  \\
SCI (5w) & 0.71 & 0.37 & 0.79 & 0.73 & 0.75 & 0.80 & 1.00 & 0.68 & 0.57  \\
CWCD (10w) & 0.55 & 0.80 & 0.55 & 0.67 & 0.65 & 0.46 & 0.68 & 1.00 & 0.62  \\
MCD (doclen) & 0.83 & 0.76 & 0.74 & 0.77 & 0.84 & 0.67 & 0.57 & 0.62 & 1.00  \\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for WordSim353 Dataset}
\label{Wordsim353CorrlMatrix}
\end{table}

\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (5s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (20w)\end{sideways} & \begin{sideways}Ochiai (25w)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (15w)\end{sideways} & \begin{sideways}CWCD (15w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways} \\
\hline
CSR (5s) & 1.00 & 0.42 & 0.86 & 0.79 & 0.88 & 0.84 & 0.69 & 0.40 & 0.59 \\
PMI (15w) & 0.42 & 1.00 & 0.33 & 0.52 & 0.56 & 0.19 & 0.21 & 0.95 & 0.77 \\
LLR (5w) & 0.86 & 0.33 & 1.00 & 0.87 & 0.90 & 0.98 & 0.64 & 0.34 & 0.53 \\
Dice (20w) & 0.79 & 0.52 & 0.87 & 1.00 & 0.95 & 0.82 & 0.42 & 0.48 & 0.53 \\
Ochiai (25w) & 0.88 & 0.56 & 0.90 & 0.95 & 1.00 & 0.85 & 0.62 & 0.53 & 0.62 \\
TTest (5w) & 0.84 & 0.19 & 0.98 & 0.82 & 0.85 & 1.00 & 0.65 & 0.20 & 0.41 \\
SCI (15w) & 0.69 & 0.21 & 0.64 & 0.42 & 0.62 & 0.65 & 1.00 & 0.32 & 0.41 \\
CWCD (15w) & 0.40 & 0.95 & 0.34 & 0.48 & 0.53 & 0.20 & 0.32 & 1.00 & 0.77 \\
MCD (doclen) & 0.59 & 0.77 & 0.53 & 0.53 & 0.62 & 0.41 & 0.41 & 0.77 & 1.00 \\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for ESSLLI Dataset}
\label{EsslliCorrlMatrix}
\end{table}



%\begin{table}
%\small\addtolength{\tabcolsep}{-3pt}
%\begin{tabular}{l c c c}\hline   
%Method    & Overall & Similarity & Relatedness \\ \hline
%CSR & 0.62 & 0.66 & 0.63\\
%WN30g & 0.66 & 0.72 & 0.56 \\
%BoW & 0.65 & 0.70 & 0.62 \\
%CW & 0.60  & 0.77  & 0.46  \\ \hline
%\end{tabular}
%\caption{ \small Comparison with previous work for Similarity, Relatedness and WordSim353 }
%\label{relsimTable}
%\end{table}


\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{p{3cm} l l}   
 \hline
Method & Source & Correlation\\
\hline
CSR (5s) & Wikipedia (April 2008) & 0.60 \\
WN30g & XXX & 0.66 \\
BoW & XXX & 0.65 \\ 
CW & XXX & 0.60  \\ 
Strube and Ponzetto, 2006 & Wikipedia & 0.19-0.48 \\
Jarmasz, 2003 &  WordNet & 0.33-0.35 \\
Jarmasz, 2003 & Roget's & 0.55 \\
Hughes and Ramage, 2007 & WordNet & 0.55 \\
Finkelstein et al., 2002 & Web corpus, WN & 0.56 \\
%(Gabrilovich and Markovitch, 2007) & ODP & 0.65 \\
Gabrilovich and Markovitch, 2007 (reimplemented in [REF]) & Wikipedia& 0.75 \\
\hline
\end{tabular}
\caption{ \small Comparison with previous work for WordSim353 }
\label{prevWorkTable}
\end{table}



\begin{table}
\small 
\begin{tabular}{|l| l| l |l| l| l|}   
 \hline
Method & Formula & \begin{sideways}Symmetry \end{sideways} & \begin{sideways}Null Addition \end{sideways}& \begin{sideways}Inversion \end{sideways}& \begin{sideways}Homogenity \end{sideways}\\
\hline
CSR &  & Y & Y & N & N\\ \hline 
LLR & $N\left(\sum_{i,j} p(i,j)log\frac{p(i,j)}{p(i)p(j)}\right)$ & Y & N & Y & Y \\ \hline
PMI & $\frac{p(x,y)}{p(x)p(y)}$ & Y & Y & N & Y \\ \hline
SCI & $\frac{p(x)p(y)}{p(x)\sqrt{p(y)}}$ & N & Y  & N  & Y\\ \hline
CWCD & $\frac{\hat{f}(x,y)}{p(x)}\frac{1/max\left(p(x),p(y)\right)}{M}$ & N & Y  & N & Y\\ \hline
MCD &  $1/M $  & X & X & X & X\\ \hline
Pearson's $\chi^2$ test & $\sum_{i,j} \frac{\left(\hat{f}(i,j)-E\hat{f}(i,j)\right)^2}{E\hat{f}(i,j)}$ & Y & N & Y & Y\\ \hline
T-test & $\frac{\hat{f}(x,y)-E\hat{f}(x,y)}{\sqrt{\hat{f}(x,y)\left(1-\frac{\hat{f}(x,y)}{N}\right)}}$ & Y & Y & N & Y\\ \hline
Dice & $\frac{2\hat{f}(x,y)}{f(x)+f(y)}$ & Y & Y & N & Y\\ \hline
Ochiai & $\frac{\hat{f}(x,y)}{\sqrt{f(x)f(y)}}$ & Y & Y & N & Y\\ \hline
Jaccard & $\frac{\hat{f}(x,y)}{f(x)+f(y)-\hat{f}(x,y)}$ & Y & Y & N & Y \\ \hline
\end{tabular}
\small
Terminology: \\
\scalebox{0.8}{%
\begin{tabular}{l l }   
$\hat{f}(x,y)$ & Constrained bigram frequency\\
$N$ & Total number of tokens in the corpus \\
$p(x,y)$ & $\hat{f}(x,y)/N $\\
$M$ & Harmonic mean of the spans of $\hat{f}(x,y)$ occurrences\\
$E\hat{f}(i,j)$ & Expected value of f(i,j): $\left(p(i)/N\right) \times \left(p(j)/N\right) \times N$ \\
$f(x)$ & frequency of $x$ in the corpus \\
\hline
\end{tabular}
}
\caption{ \small Properties of methods }
\label{methods}
\end{table}

\clearpage

